A Robust Riemann Solver for Multiple Hydro-Elastoplastic Solid Mediums

We propose a robust approximate solver for the hydro-elastoplastic solid material, a general constitutive law extensively applied in explosion and high speed impact dynamics, and provide a natural transformation between the fluid and solid in the case of phase transitions. The hydrostatic components of the solid is described by a family of general Mie-Gr\"uneisen equation of state (EOS), while the deviatoric component includes the elastic phase, linearly hardened plastic phase and fluid phase. The approximate solver provides the interface stress and normal velocity by an iterative method. The well-posedness and convergence of our solver are proved with mild assumptions on the equations of state. The proposed solver is applied in computing the numerical flux at the phase interface for our compressible multi-medium flow simulation on Eulerian girds. Several numerical examples, including Riemann problems, shock-bubble interactions, implosions and high speed impact applications, are presented to validate the approximate solver.

==> mp_intro.tex <==
\begin{abstract}
We propose a robust approximate solver for the hydrodynamic elastoplastic solid
material, which is a general constitutive law extensively applied in explosion
and impact dynamics. 

\end{abstract}

\begin{keyword}

\end{keyword}
\maketitle


\section{Introduction}
Significant interest has arisen in the modeling and simulation of dynamic 
events that involve high-load conditions and large deformations, such as 
shock-driven motions, high-speed impacts, implosions, and so on. The numerical 
analysis of these problems demands the implementation of very specific 
capabilities that enable the simulation of multiple materials and their 
interaction through accurate descriptions of boundary condtions and 
high-resolution shock and wave capturing. 

There are two typical frameworks to describe the motion of multi-medium flows
\cite{Benson1992}, that is, the Lagrangian framework and the Eulerian 
framework. In Lagrangian framework, the equations for mass, momentum and energy 
conservations are solved using a computational mesh that conforms to the 
material boundaries and moves with particles \cite{Camacho1997adaptive, 
Bessette2003modeling}, which benifits from its simplicity and natural 
description of deformation, but suffers from mesh distortion when dealing with 
large deformation problems. In Eulerian framework the mesh is fixed in space, 
which makes these methods very suitable for flows with large deformations, such 
as Udaykumar \textit{et al.} \cite{Udaykumar1997, Tran2004, Udaykumar2003, 
Sambasivan2011, Sambasivan2013, Kapahi2013}, Liu \textit{et al.} \cite{Wang2009, 
Wang2007, Wang2010, Chen2012, Chen2010, Hua2011}, Mehmandoust \textit{et al.} 
\cite{Mehmandoust2009}, Sijoy \textit{et al.} \cite{Sijoy2015}, and so on. A 
typical procedure of fluid-solid interaction in Eulerian grids mainly consists 
of two steps. The first step is the interface capture, including the diffuse 
interface method (DIM) \cite{Abgrall1996, Abgrall2001, Saurel1999, Saurel2009, 
Petitpas2009, Ansari2013}, and the sharp interface method (SIM) including the 
volume of fluid (VOF) method \cite{Scardovelli1999, Noh1976}, level set method 
\cite{Sethian2001, Sussman1994}, moment of fluid (MOF) method \cite{Ahn2007, 
Dyadechko2008, Anbarlooei2009} and front-tracking method \cite{Glimm1998, 
Tryggvason2001}. The second step is the accurate prediction of the interface 
states, which can be used to stabilize the numerical diffusion in diffuse 
interface methods, and to compute the numerical flux and interface motion in 
sharp interface methods. One common approach is to solve a multi-medium Riemann 
problem which contains the fundamentally physical and mathematical properties of 
the governing equations and plays a key role in designing the numerical flux. 


The solution of a multi-medium Riemann problem depends not only on the initial
states at each side of the interface, but also on the forms of equations of
state. There exist some difficulties in the cases of general nonlinear equations 
of state due to their high nonlinearity. A variety of methods to solve the 
corresponding Riemann problems have then been proposed. For example, 
Yadav \cite{Yadav1982converging} analyzed spherical shocks in metals employing 
a hydrostatic Mie-Gr{\"u}neisen EOS that does not reflect the effects of shear 
deformation. Shyue \cite{Shyue2001} developed a Roe's approximate Riemann solver 
for the Mie-Gr{\"u}neisen EOS with variable Gr{\"u}neisen coefficient. Arienti 
\textit{et al.} \cite{Arienti2004} applied a Roe-Glaster solver to compute the
equations combining the Euler equations involving chemical reaction with the
Mie-Gr{\"u}neisen EOS. Lee \textit{et al.} \cite{Lee2013} developed an exact 
Riemann solver for the Mie-Gr{\"u}neisen EOS with constant Gr{\"u}neisen 
coefficient, where the integral terms are evaluated using an iterative Romberg 
algorithm. Banks \cite{Banks2010} and Kamm \cite{Kamm2015} developed a Riemann 
solver for the convex Mie-Gr{\"u}neisen EOS by solving a nonlinear equation for 
the density increment involved in the numerical integration of rarefaction 
curves. Unlike the fluid, there may exist more than one nonlinear wave in a 
solid when it undergoes an elastoplastic deformation, which will increase the 
difficulty to obtain the exact solution of the fluid-solid Riemann problem. 
Several methods have been studied to solve the above problems. Kaboudian 
\textit{et al.} \cite{Kaboudian2014} analyzed the elastic Riemann problem in the 
Lagrangian framework, and established the corresponding Riemann solver according 
to the characteristic theory, where the constitutive equation was the Hooke's 
law for one-dimensional isotropic linearly elastic solid. Xiao \textit{et al.} 
\cite{Xiao1996} raised an iterative procedure to solve the Riemann problem 
approximately by linearizing the Riemann invariants. Tang \textit{et al.} 
\cite{Tang1999} put forward a nearly exact Riemann solver for the 
hydro-elastoplastic solid based on the physical observation, where the Murnagham 
equation of state (EOS) and perfect plasticity model were chosen for the 
hydrostatic pressure and deviatoric stress respectively. Abouziarov \textit{et 
al.} \cite{Abouziarov2000} and Bazhenov \textit{et al.} \cite{Bazhenov2002} 
analyzed the structures of shock waves and rarefaction waves in an elastoplastic 
material on the assumption of barotropy, without taking into account the 
internal energy equation. Cheng \textit{et al.} \cite{Chen2012, Chen2010} 
analyzed the wave structures of one-dimensional elastoplastic flows and 
developed a two-rarefaction approximate Riemann solver (TRRSE). Menshov 
\textit{et al.} \cite{Menshov2014} provided an analysis of the Riemann problem 
in a complete statement for the perfect plasticity on the assumption of 
one-dimensional motion and uniaxial strain. Lin \textit{et al.} \cite{Lin1993} 
established a Riemann solver for the one-dimensional longitudinal and torsional 
stress wave problem of the thin-walled elastoplastic tube. Trangenstein 
\textit{et al.} \cite{Trangenstein1991a} constructed the analytical solution of 
the Riemann problem for the Antman--Szymczak model of longitudinal motion in an 
elastoplastic bar. Liu \textit{et al.} \cite{Liu2008, Liu2011}, Feng \textit{et 
al.} \cite{Feng2017} and Gao \textit{et al.} \cite{Gao2017, Gao2018} analyzed 
the exact solution of the elastic-perfectly plastic solid with the Murnagham EOS 
and stiffened gas EOS, and combined it with the modified ghost fluid method to 
solve multi-medium problems. Gavirilyuk \textit{et al.} \cite{Gavrilyuk2008} 
constructed a Riemann solver for the linearly elastic system of the hyperbolic 
non-conservative models with transverse waves. In addition, the elastic energy 
was included in the total energy, and an extra evolution equation, on the basis 
of Despres \textit{et al.} \cite{Despres2007}, was added in order to make the 
elastic transformation reversible in the absence of shock wave. Kamm \textit{et 
al.} \cite{Kamm2014} reviewed and validated Gavirilyuk's work by using the FLAG 
code, and gave a qualitative analysis of the comparison. 


In this paper, we develop an approximate fluid-solid Riemann solver with a 
family of general Mie-Gr{\"u}neisen EOS and hydrodynamic elastoplastic 
deviatoric deformation, which can provide a smooth transition between fluid 
and solid in the case of phase changes. The Riemann problem together with its 
approximate solver in such case, which has not been well studied in the 
literature yet, can be applied in the numerical scheme developed in 
\cite{Guo2016} conveniently. The study we carried out here is a further 
exploration of our previous work in \cite{Lichen2018}, which is restricted on 
the fluid-fluid Riemann solver with Mie-Gr{\"u}neisen EOS. Similar to the solver 
in \cite{Lichen2018}, some mild conditions on the coefficients of 
Mie-Gr{\"u}neisen EOS are assumed to ensure the convexity of the equation of 
state, which guarantees the existence and uniqueness of the algebraic equation 
derived from the Riemann problem. The algebraic equation is derived by a 
detailed analysis on the structure of the Riemann fan. Then we solve the 
algebraic equation by an inexact Newton method \cite{Dembo1982}, where the 
function and its derivatives are evaluated approximately since the analytical 
expressions are not available. The approximate evaluations of the function and 
its derivatives are quite involved since they depend on the wave structure and 
the error estimate in the run time. In spite of its complexity, we find that the 
convergence of the inexact Newton iteration can be achieved, which is 
significant to the success of large-scale simulations in engineering 
applications. To validate the proposed approximate Riemann solver, we employ it 
in the computation of multi-medium compressible flows with Mie-Gr{\"u}neisen EOS 
and elastoplastic deformation. The approximate solver developed here enhances 
the capacity of the numerical scheme for our multi-medium compressible fluid 
flows \cite{Guo2016, Lichen2018}, and allows us to simulate the problems with 
practical elastoplastic solid materials.

The rest of this paper is arranged as follows. In Section \ref{sec:rp}, a
solution strategy for the multi-medium Riemann problem with Mie-Gr{\"u}neisen
EOS and hydrodynamic elastoplastic deviatoric deformation is presented. In 
Section \ref{sec:aps}, the procedures of our approximate Riemann solver are 
outlined, and the well-posedness and convergence are analyzed. In Section 
\ref{sec:sch}, the application of our Riemann solver in multi-medium 
compressible flow calculations is briefly introduced. In Section \ref{sec:num}, 
several classical Riemann problems and applications for surface blast, 
subsurface blast and high speed impact problems are carried out to validate the 
accuracy and robustness of our methods. Finally, a short conclusion is drawn in 
Section \ref{sec:conclusion}.




The hydrodynamic elastoplastic solid can degenerate to elasticity,
elastoplasticity and fluid dynamics. 

In high-rate and large deformation region, the volumeric deformation is
dominant and the deviatoric deformation can be neglected. When the load is
removed, the elastoplastic effect should be taken into account again. 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 


==> mp_result.tex <==
\section{Numerical examples}\label{sec:num}

In this section we present some numerical examples to validate our methods,
including one-dimensional Riemann problems, spherically symmetric problems and
two-dimensional shock impact problems. One-dimensional and spherically
symmetric simulations are carried out on uniform interval meshes, while
two-dimensional simulations are carried out on unstructured triangular meshes. 

\subsection{One-dimensional Riemann problems}

In this part, we present some numerical examples of one-dimensional Riemann
problems. The computational domain is $[0,1]$ with $400$ cells, and both the
left and right boundaries are set as outflow conditions. The reference
solutions, if mentioned, are given from either published results or computed on
a very fine mesh with $10^4$ cells.

\subsubsection{Gas-gas Riemann problem}
In the first example, we study a single-phase problem from \cite{Toro2008},
where a standard Eulerian scheme also works well with no oscillation. We take it
as a two-phase problem by artifically embedding an interface at $x=0.5$
initially. The initial values are 
\[
[\rho, u, p]^\top = \left\{
\begin{array}{ll}
[1.0, ~0, ~10^3]^\top,     &x<0.5,\\ [2mm]
[1.0, ~0, ~10^{-2}]^\top, & x > 0.5.
\end{array}
\right.
\]

\begin{figure}[htbp]
\centering
\subfloat[Density]
{\includegraphics[width=0.3\textwidth]{gas-gas/dens.eps}}
\subfloat[Pressure]
{\includegraphics[width=0.3\textwidth] {gas-gas/p.eps}}
\subfloat[Velocity]
{\includegraphics[width=0.3\textwidth]{gas-gas/vel.eps}} 
\caption{Gas-gas Riemann problem.}
\label{res:gas-gas}
\end{figure}

We carry out the simulation to a final time of 0.012. Fig. \ref{res:gas-gas}
shows the comparison between the numerical results and the exact solutions.
From the comparison we can see that the numerical results behave in perfect
agreement with the exact solutions. 


\subsubsection{JWL-polynomial Riemann problem}
\label{sec:jwl-water}
This example concerns the JWL-polynomial Riemann problem. The initial states
are 
\[
[\rho, u, p]^\top = \left\{
\begin{array}{ll}
[1630, ~0, ~8.3\times 10^9]^\top, &x<0.5,\\ [2mm]
[1000, ~0, ~1.0\times 10^5]^\top, & x > 0.5.
\end{array}
\right.
\]
We use the following values to describe the TNT \cite{Smith1999}:
$A_1=\unit[3.712\times10^{11}]{Pa}$,
$A_2=\unit[3.230\times10^9]{Pa}$,
$\omega=0.30$, 
$R_1=4.15$, 
$R_2=0.95$ and $\rho_0=\unit[1630]{kg/m^3}$. 
The parameters of the polynomial EOS are 
$\rho_0=\unit[1000]{kg/m^3}$,
$A_1=\unit[2.20\times10^9]{Pa}$, $A_2=\unit[9.54\times10^9]{Pa}$,
$A_3=\unit[1.45\times10^{10}]{Pa}$, $B_0=B_1=0.28$, 
$T_1=\unit[2.20\times10^9]{Pa}$ and $T_2=0$ for the
polynomial EOS \cite{Jha2014}. 

\begin{figure}[htbp]
\centering
\subfloat[Density]
{\includegraphics[width=0.3\textwidth]{jwl-poly/dens.eps}}
\subfloat[Pressure]
{\includegraphics[width=0.3\textwidth] {jwl-poly/p.eps}}
\subfloat[Velocity]
{\includegraphics[width=0.3\textwidth]{jwl-poly/vel.eps}} 
\caption{Gas-gas Riemann problem.}
\label{res:jwl-ploy}
\end{figure}


The result at $t=8.0\times 10^{-5}$ is shown in Fig. \ref{res:jwl-ploy}, where
we can observe that both the interface and shock are captured well without
spurious oscillation. 



\subsubsection{Gavrilyuk elastic solid Riemann problem}
\label{sec:e-e}
In this problem, we simulate an elastic solid-solid Riemann problem
\cite{Gavrilyuk2008}. The hydrostatic presure of the solid is described by the
stiffened gas EOS with parameters $\gamma=4.4$, $p_\infty=6\times 10^6$Pa.
And the deviatoric component obeys the Hooke's law, where the elastic shear
modulus is $\mu^{_\mathscr E}=10^{10}$Pa. The initial values are given by
\[
 [\rho, u, p]^\top = \left\{
  \begin{array}{ll}
    [10^3, ~100, ~10^5]^\top, & x < 0.5,\\[2mm]
    [10^3, ~-100, ~10^5]^\top, & x > 0.5.
  \end{array}
 \right.
\]

The comparison between our numerical results and reference solutions at
$6.1\times 10^{-5}$ is shown in Fig. \ref{res:e-e}. Each solid has two
nonlinear waves, the leading elastic shock wave and trailing plastic shock
wave, and there is no oscillation in the vicinity of phase interface and shock
waves.

\begin{figure}[htbp]
\centering
\subfloat[密度]
{\includegraphics[width=0.3\textwidth]
  {e-e/dens.eps}}
\subfloat[应力]
{\includegraphics[width=0.3\textwidth] 
  {e-e/p.eps}}
\subfloat[速度]
{\includegraphics[width=0.3\textwidth]
  {e-e/vel.eps}} \\
%------------------------------------
%\addtocounter{subfloat}{-3}
\subfloat
{\includegraphics[width=0.3\textwidth]
  {e-e/dens-ref.png}}
\quad
\subfloat
{\includegraphics[width=0.29\textwidth]
  {e-e/p-ref.png}}
\quad
\subfloat
{\includegraphics[width=0.29\textwidth]
  {e-e/vel-ref.png}} \\
\caption{Gavrilyuk elastic solid Riemann problem (top row: our results, bottom
row: results from Gavrilyuk \textit{et al.} \cite{Gavrilyuk2008}).} 
\label{res:e-e}
\end{figure}


\subsubsection{JWL-elastic solid Riemann problem}
\label{res:jwl-elastic}
In this problem, we simulate a JWL-elastic solid Riemann problem. The JWL
EOS has the same parameters as that in Section \ref{sec:jwl-water}, and the
elastic solid has the same constitutive law  as Section \ref{sec:e-e} with
$\beta^{_\mathscr E}=10^{14}~\mbox{Pa}\cdot\mbox{kg/m}^3$. The initial values
are
\[
 [\rho, u, p]^\top = \left\{
  \begin{array}{ll}
    [1630, ~0, ~9.2\times 10^9]^\top, & x < 0.5, \\ [2mm]
    [7800, ~0, ~10^5]^\top, & x > 0.5.
  \end{array}
 \right.
\]

\begin{figure}[htbp]
\centering
\subfloat[Density]
{\includegraphics[width=0.3\textwidth]{jwl-e/dens.eps}}
\subfloat[Pressure]
{\includegraphics[width=0.3\textwidth] {jwl-e/p.eps}}
\subfloat[Velocity]
{\includegraphics[width=0.3\textwidth]{jwl-e/vel.eps}} 
\caption{JWL-elastic solid Riemann problem.}
\label{res:jwl-e}
\end{figure}

The computation terminates at $10^{-4}$. Fig. \ref{res:jwl-e} displays the
results of our numerical scheme and the exact solutions, where we can see that
there is no non-physical pressure and velocity across the contact discontinuity
in our numerical scheme.



\subsubsection{Elastoplastic-elastoplastic solid Riemann problem}
\label{sec:ep-ep}
In this problem, we simulate a elastoplastic-elastoplastic solid Riemann
problem. We set the following parameters for the solid: $\mu^{_\mathscr
E}=\unit[8.53\times 10^5]{Pa},~ \mu^{_\mathscr P}=0,~ K=\unit[2.225\times
10^6]{Pa},~ Y=\unit[6.50\times 10^3]{Pa}$. 
The initial values are given by
\[
 [\rho, u, p, \gamma]^\top = \left\{
  \begin{array}{ll}
    [3.0, ~0, ~10^{5},~ 2.0]^\top, & x < 0.4,\\[2mm]
    [7.8, ~0, ~1.0,~ 3.7]^\top, & x > 0.4.
  \end{array}
 \right.
\]


\subsection{Spherically symmetric problems}
In this part we consider two spherically symmetric Riemann problems, where the
governing equations are formulated as 
\begin{equation}
\pdd t
\begin{pmatrix}
r^2\rho \\ r^2\rho u \\ r^2E
\end{pmatrix}
+\pdd r
\begin{pmatrix}
r^2\rho u \\ r^2(\rho u^2+p-S_r) \\ r^2(E+p)u
\end{pmatrix}
=\begin{pmatrix}
0 \\ 2rp \\ 0
\end{pmatrix}.
\label{eq:spheq}
\end{equation}
The source term in \eqref{eq:spheq} is discretized using an explicit Euler
method, where $p$ is the pressure.

We first consider two fluid-solid Riemann problem in spherical coordinates,
which have the same constitutive law and initial conditions as Section
\ref{sec:jwl-water} and \ref{res:jwl-e}, respectively. The
computational domain is $[0,1]$ with $400$ cells, and both the left and right
boundaries are set as outflow conditions. 

\begin{figure}[htbp]
\centering
\subfloat[Density]
{\includegraphics[width=0.3\textwidth]
{jwl-stiff-sphere/dens.eps}}
\subfloat[Pressure]
{\includegraphics[width=0.3\textwidth]
{jwl-stiff-sphere/p.eps}}
\subfloat[Velocity]
{\includegraphics[width=0.3\textwidth]
{jwl-stiff-sphere/vel.eps}}
\caption{Spherical JWL-stiffened gas Riemann problem.}
\label{res:jwl-stiff-sph}
%--------------------------------
\subfloat[Density]
{\includegraphics[width=0.3\textwidth]
{jwl-poly-sphere/dens.eps}}
\subfloat[Pressure]
{\includegraphics[width=0.3\textwidth]
{jwl-poly-sphere/p.eps}}
\subfloat[Velocity]
{\includegraphics[width=0.3\textwidth]
{jwl-poly-sphere/vel.eps}}
\caption{Spherical JWL-polynomial Riemann problem.}
\label{res:rm_jwl_pol_sph}
\end{figure}


From Fig. \ref{res:jwl-stiff-sph} and \ref{res:rm_jwl_pol_sph} we can see that
the numerical results agree well with the reference solutions computed on a very
fine mesh with $10^4$ cells. The results also exhibit high resolution in the
vicinity of shock waves and contact discontinuity. Due to the presence of the
geometric source term, the states in the star region are no longer uniform.



\subsection{Two-dimensional applications}

In this part, we present a few two-dimensional problems in engineering
applications, which are carried out on triangular meshes. All of the physical
boundaries are set as outflow boundary conditions.

\subsubsection{Gas-bubble interaction problem}
In this problem, we simulate a gas-bubble problem from Hass
\cite{Haas1987interaction}.
%\cite{Haas1987interaction, ullah2013towards, quirk1996dynamics}.

\begin{figure}[htbp]
\centering
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/a.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/23us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/b.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/43us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/c.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/53us-1.png}} \\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/d.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/66us-1.png}} \\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/e.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/75us-1.png}} 
\caption{Gas-bubble interaction problem. 
The first row: 32$\mu\mbox{s}$,~53$\mu\mbox{s}$,
62$\mu\mbox{s}$,~72$\mu\mbox{s}$, 82$\mu\mbox{s}$;~
The second row: 23$\mu\mbox{s}$,~43$\mu\mbox{s}$,
53$\mu\mbox{s}$,~66$\mu\mbox{s}$, 75$\mu\mbox{s}$.}
\label{res:shock-bubble1}
\end{figure}


\begin{figure}[htbp]
\centering
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/f.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/102us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/g.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/260us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/h.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/445us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/i.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/674us-1.png}}\\
\vspace{5mm}
\subfloat
{\includegraphics[width=0.24\textwidth]
{shock-bubble/j.png}}\quad
\subfloat
{\includegraphics[width=0.7\textwidth]
{shock-bubble/layer/983us-1.png}}
\caption{Gas-bubble interaction problem. 
The first row: 102$\mu\mbox{s}$,~245$\mu\mbox{s}$,
427$\mu\mbox{s}$,~674$\mu\mbox{s}$, 983$\mu\mbox{s}$;~
The second row: 102$\mu\mbox{s}$,~260$\mu\mbox{s}$,
445$\mu\mbox{s}$,~674$\mu\mbox{s}$, 983$\mu\mbox{s}$.}
\label{res:shock-bubble2}
\end{figure}


\subsubsection{Blast wave reflection of TNT explosion}
In this problem, we simulate a TNT explosion problem, where the blast wave
is reflected by a rigid surface near the explosion center.
\begin{figure}[htbp]
\centering
\subfloat[$t=1.0 \mu$s]
{\includegraphics[width=0.18\textwidth]
{near/60-1.png}}
\subfloat[$t=4.3 \mu$s]
{\includegraphics[width=0.181\textwidth]
{near/90-1.png}}
\subfloat[$t=3.0 \mu$s]
{\includegraphics[width=0.176\textwidth]
{near/120-1.png}} 
\subfloat[$t=7.0 \mu$s]
{\includegraphics[width=0.181\textwidth]
{near/150-1.png}}
\subfloat[$t=11.0 \mu$s]
{\includegraphics[width=0.183\textwidth]
{near/210-1.png}} \\
\caption{Pressure contours for TNT explosion problem.}
\label{res:tnt_ref_cont}
\vspace{15mm}
\subfloat[Peak overpressure]
{\includegraphics[width=0.45\textwidth]
{near/p.eps}}
\subfloat[Impulse]
{\includegraphics[width=0.45\textwidth]
{near/I.eps}}
\caption{Shock wave parameters for nuclear air blast problem.
The reference solution 1 is taken from \cite{Baker1973},
the reference solution 2 is taken from \cite{Huffington1985},
the reference solution 3 is taken from \cite{Hokanson1978}, while 
the reference solution 3 is taken from \cite{Zhangdz2009}. }
\label{res:tnt_ref}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Implosion compression problem}
We consider a two dimensional problem of implosion compression, which is
applied widely in inertial confinement fusion \cite{Jia2014}. 
The initial shape of the model is a sphere, which contains three distinct
mediums, TNT, tungsten and air. The outmost layer is the high explosive products
of TNT , which is described by the JWL EOS with parameters
$A_1=\unit[8.524\times10^{11}]{Pa}$, $A_2=\unit[1.802\times10^{10}]{Pa}$,
$\omega=0.38$, $R_1=4.6$, $R_2=1.3$, 
$\rho_0=\unit[1842]{kg/m^3}$. The intermediate layer is the tungsten, which is
described by the stiffened gas EOS with parameters $\gamma=4.075$,
$\rho_0=7.85~\mbox{g/cm}^3$. The innermost layer is the air, which is described
by the ideal gas with $\gamma=1.4$. The initial values are 

\[
 [\rho, u, p]^\top = \left\{
  \begin{array}{ll}
    [1.29, ~0, ~10^5]^\top, & r < 0.1, \\ [2mm]
    [1.9237\times 10^4, ~0, ~10^5]^\top, & 0.1 \le r \le 0.105, \\ [2mm]
    [1.63\times 10^3, ~0, ~10^5]^\top, & 0.105 < r < 0.12, \\ [2mm]
  \end{array}
 \right.
\]

\iffalse
\begin{figure}[htbp]
\centering
{\includegraphics[width=0.5\textwidth]
{icf/icf.png}}
\caption{Model of implosion explosion.}
\label{res:icf_mode}
\end{figure}
\fi




\begin{figure}[htbp]
\centering
\subfloat[$10\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/10us-1.png}} 
\subfloat[$20\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/20us-1.png}} \\
\vspace{5mm}
\subfloat[$30\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/30us-1.png}}
\subfloat[$32\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/32us-1.png}} \\
\vspace{5mm}
\subfloat[$34\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/34us-1.png}} 
\subfloat[$36\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/36us-1.png}}
\caption{Pressure contours for implosion compression problems. }
\label{res:icf1}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[$37\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/37us-1.png}} 
\subfloat[$37.2\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/37.2us-1.png}} \\
\vspace{5mm}
\subfloat[$37.5\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/37.5us-1.png}}
\subfloat[$39\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/39us-1.png}} \\
\vspace{5mm}
\subfloat[$40\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/40us-1.png}} 
\subfloat[$50\times 10^{-6}~\mbox{s}$]
{\includegraphics[width=0.45\textwidth]
{icf/50us-1.png}}
\caption{Pressure contours for implosion compression problems. }
\label{res:icf2}
\end{figure}




\subsection{Three-dimensional applications}
In this problem, we simulate a three dimensional high speed impact problem
between two elastoplastic solids. A cylindrical rod made of steel with an
initial radius of $\unit[0.0025]{m}$ is given a velocity of $\unit[7000]{m/s}$
and impacts against a static alumnium, shown as Fig. \ref{res:impact} (a). The
alumnium has an initial radius of $\unit[0.02]{m}$ and a length of
$\unit[0.01]{m}$. In fact, the whole problem involves three mediums, the steel,
the alumnium and the air. The equations of state of the hydrostatic pressure
component for the steel and alumnium are both taken as the stiffened gas EOS,
and the deviatoric component are both taken as the perfect plasticity. The
intial parameters are 
$\rho_0=\unit[7840]{kg/m^3}$, $\gamma=4.075$,
$\mu^{_\mathscr E}=\unit[78.5\times10^9]{Pa}$, $\mu^{_\mathscr P}=0$, 
$Y=\unit[160\times10^6]{Pa}$ for the steel, 
and $\rho_0=\unit[2790]{kg/m^3}$, $\gamma=2.75$, 
$\mu^{_\mathscr E}=\unit[27.4\times10^9]{Pa}$, $\mu^{_\mathscr P}=0$, 
$Y=\unit[34\times10^6]{Pa}$ for the alumnium. The air is modeled
by the ideal gas EOS with the following initial parameters:
$\rho_0=\unit[1.29]{kg/m^3}$,
$\gamma=1.4$ and $p_0=\unit[1.013\times10^5]{Pa}$. 

Fig. \ref{res:impact} (b)--(f) show the density contours of the whole steel and
alumnium at different time. When the steel rod reaches the alumnium, strong
interaction occurs between them. Since the steel has a much higher density and
stiffness, it will lead to the severe deformation and penetration of the
alumnium finally. In the whole calculation, we can see that the interfaces
between each pair of the alumnium, steel and air can be captured sharply,
which show that our numerical scheme can handle the large deformation of
compressible materials and phase interfaces naturally.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 

